MSeg: A Composite Dataset for Multi-domain Semantic Segmentation

We present MSeg, a composite dataset that unifies semantic segmentation datasets from different domains. A naive merge of the constituent datasets yields poor performance due to inconsistent taxonomies and annotation practices. We reconcile the taxonomies and bring the pixel-level annotations into alignment by relabeling more than 220,000 object masks in more than 80,000 images, requiring more than 1.34 years of collective annotator effort. The resulting composite dataset enables training a single semantic segmentation model that functions effectively across domains and generalizes to datasets that were not seen during training. We adopt zero-shot cross-dataset transfer as a benchmark to systematically evaluate a model's robustness and show that MSeg training yields substantially more robust models in comparison to training on individual datasets or naive mixing of datasets without the presented contributions. A model trained on MSeg ranks first on the WildDash-v1 leaderboard for robust semantic segmentation, with no exposure to WildDash data during training. We evaluate our models in the 2020 Robust Vision Challenge (RVC) as an extreme generalization experiment. MSeg training sets include only three of the seven datasets in the RVC; more importantly, the evaluation taxonomy of RVC is different and more detailed. Surprisingly, our model shows competitive performance and ranks second. To evaluate how close we are to the grand aim of robust, efficient, and complete scene understanding, we go beyond semantic segmentation by training instance segmentation and panoptic segmentation models using our dataset. Moreover, we also evaluate various engineering design decisions and metrics, including resolution and computational efficiency. Although our models are far from this grand aim, our comprehensive evaluation is crucial for progress. We share all the models and code with the community.

==> classdefinitions.tex <==
\onecolumn
% \begin{portrait}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\renewcommand{\arraystretch}{0.81}
\scriptsize
\begin{longtable}{@{}p{20mm}@{\hspace{5mm}}p{4cm}@{\hspace{1cm}}l@{}}
\caption[Landscape multiple page table]{Comprehensive MSeg class list: definitions and examples }
\label{tab:classdefs} \\
\toprule \\
\textbf{Universal} & \textbf{Description} & \textbf{Examples} \\
\textbf{Class Name} & & \\
\\
\midrule \\
\endfirsthead
\multicolumn{3}{c}{{\tablename} \thetable{} -- Continued}\\%[0.5ex]
\toprule \\%[-2ex]
\textbf{Universal} & \textbf{Description} & \textbf{Examples} \\
\textbf{Class Name} & & \\
\\
    \midrule \\%[-2ex]
\endhead
\midrule \\
\multicolumn{3}{c}{{Continued on Next Page\ldots}} \\
\endfoot \\
\endlastfoot
% \multirow{15}{*}{\begin{sideways}{\Large{1\% gas}}\end{sideways}}
% Class 1 & This Class is blah & . Picture\\[0.3ex]\hline\\[0.3ex]
% \multirow{15}{*}{\begin{sideways}{\Large{10\% gas}}\end{sideways}}
 airplane & an aircraft that has a fixed wing and is powered by propellers or jets &
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/airplane1_val2017_000000497568.jpeg}} \\
 animal-other & Any animal that is not a bird, cat, dog, horse, sheep, cow, elephant, bear, zebra, or giraffe  & \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/animal-other1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/animal-other2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/animal-other3.jpeg}}\\
 apparel & clothing in general, not currently being worn by a human being & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/apparel1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/apparel2.jpeg}}\\
 apple & fruit with red or yellow or green skin and sweet to tart crisp whitish flesh & \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/apple1.jpeg}} \\
 arcade machine & & \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/arcade_machine1.jpeg}} \\
 armchair & chair with a support on each side for arms (that is not a swivel chair, seat, or sofa) & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/armchair2.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/armchair3.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/armchair6.jpeg}} \\

autorickshaw & in South Asia, a small motor vehicle with three wheels that is used as a taxi & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/autorickshaw2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/autorickshaw1.jpeg}}
\\
 awning & a sheet of canvas or other material stretched on a frame and used to keep the sun or rain off a storefront, window, doorway, or deck. Should be attached to a building. & \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/awning1.jpeg}} \\
 backpack & a bag carried by a strap on your back or shoulder & \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/backpack2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/backpack1.jpeg}} \\
 bag & & \\
 banana & elongated crescent-shaped yellow fruit with soft sweet flesh & \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/banana1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/banana2.jpeg}} \\
 banner & long strip of cloth or paper used for decoration or advertising & \\
 barrel & a cylindrical container that holds liquids & \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/barrel1.jpeg}} \\
 base & & \\
 baseball bat & an implement used in baseball by the batter & \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/baseballbat1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/baseballbat2.jpeg}} \\
 baseball glove & the handwear used by fielders in playing baseball & \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/baseballglove1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/baseballglove2.jpeg}} \\
 basket & a container used to hold or carry things, typically made from interwoven strips of cane or wire. & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/basket1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/basket2.jpeg}}\\
 bathtub & & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/bathtub1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bathtub2.jpeg}} \\
 bathroom-counter & a long, flat, narrow surface in a bathroom at waist-height & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/bathroom-counter1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bathroom-counter2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bathroom-counter3.jpeg}} \\
bathtub & & \\
 bear & massive plantigrade carnivorous or omnivorous mammals with long shaggy coats and strong claws &
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/bear1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bear2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bear3.jpeg}} \\
 bed & & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/bed1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bed2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bed3.jpeg}} \\
 bench & a long seat for more than one person & 
 \raisebox{-.5\height}{
 \includegraphics[height=1.7cm]{latex/classdefimgs/bench1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bench2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bench3.jpeg}}\\
 bicycle & a wheeled vehicle that has two wheels and is moved by foot pedals & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/bicycle1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bicycle2.jpeg}}\\
 bicyclist & a person who rides a bicycle & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/bicyclist1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bicyclist2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bicyclist3.jpeg}}\\
 bike rack & a rack for parking bicycles & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/bikerack1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bikerack2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bikerack3.jpeg}}\\
 billboard & & \\
 bird & warm-blooded egg-laying vertebrates characterized by feathers and forelimbs modified as wings & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/bird_example1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bird_example2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bird4.jpeg}}\\
 blanket & & \\
 boat-ship & & \\
 book & & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/book1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/book2.jpeg}}\\

 bookshelf & & \\

 bottle & a glass or plastic vessel used for storing drinks or other liquids; typically cylindrical without handles and with a narrow neck that can be plugged or capped & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/bottle1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bottle2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bottle3.jpeg}} \\
 \\

 bowl &  & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/bowl1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bowl2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bowl3.jpeg}} \\
% \textcolor{red}{Note: COCO inconsistent about bowl contents} & & \\

 box & & \\

 bridge & a structure that allows people or vehicles to cross an obstacle such as a river or canal or railway etc. & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/bridge1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bridge2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bridge3.jpeg}} \\

 broccoli & plant with dense clusters of tight green flower buds &
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/broccoli1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/broccoli2.jpeg}} \\

 building & a structure that has a roof and walls and stands more or less permanently in one place. Includes houses, grandstands, booths, towers, and skyscrapers. & \\

 bulletin board & & \\

 bus & a large vehicle carrying many passengers; used for public transport. Typically has swing doors, more than 4 wheels, tires larger than a regular car, and an illuminated front sign &
 \raisebox{-.75\height}{
  \includegraphics[height=1.7cm]{latex/classdefimgs/bus1.jpeg}
 \includegraphics[height=1.7cm]{latex/classdefimgs/bus2.jpeg}}\\

 cabinet & A case or cupboard usually having doors and shelves. Can be found in a bathroom, kitchen, or other room. Cabinets are not for storing clothes. &
\raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/kitchen-cabinet-example-4.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/bathroom-cabinet-example-1.jpeg}}\\

 cake & baked goods made from or based on a mixture of flour, sugar, eggs, and fat & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/cake1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/cake2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/cake3.jpeg}} \\

 car & & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/car1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/car2.jpeg}}
%\includegraphics[height=1.7cm]{latex/classdefimgs/car3.jpeg}
\\

\hline
 carrot & deep orange edible root of the cultivated carrot plant & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/carrot1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/carrot2.jpeg}} \\

 case & a glass container used to store and display items in a shop or museum or home & \\

 cat & feline mammal usually having thick soft fur and no ability to roar: domestic cats & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/cat1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/cat2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/cat3.jpeg}} \\

 cctv camera & camera that can produce images or recordings for surveillance or other private purposes & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/cctvcamera1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/cctvcamera2.jpeg}} \\

 ceiling & & \\

 cell phone & a phone with access to a cellular radio system so it can be used over a wide area, without a physical connection to a network; a mobile phone. &
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/cell_phone2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/cell_phone1.jpeg}} \\

 chair\_other & Any chair that does NOT fall into the following categories: armchair, stool, seat, sofa.  A chair is defined as a seat for one person, with a support for the back. &
  \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/chair-other3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/chair-other2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/chair-other1.jpeg}} \\

 chandelier & branched lighting fixture; often ornate; hangs from the ceiling & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/chandelier1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/chandelier2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/chandelier3.jpeg}} \\

 chest of drawers & furniture with drawers for keeping clothes & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/chest-of-drawers-example-1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/chest-of-drawers-example-7.jpeg}} \\

 clock & a timepiece that shows the time of day &
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/clock1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/clock2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/clock3.jpeg}} \\

 column & (architecture) a tall vertical cylindrical structure standing upright and used to support a structure & 
\raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/column4.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/column1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/column2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/column3.jpeg} } \\

 conveyor belt & 
 a moving belt that transports people or objects (as in a factory). Includes moving walkways and baggage carousels & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/conveyorbelt3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/conveyorbelt2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/conveyorbelt1.jpeg}}
 \\

 couch & an upholstered seat for more than one person (also known as sofa) & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/couch4.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/couch3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/couch2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/couch1.jpeg}} \\

 counter-other & a long, flat, narrow surface used for making transactions in a store or in a home kitchen (fixed against a wall for preparing food). & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/counter-other1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/counter-other2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/counter-other-3.jpeg}} \\

 cow & cattle that are reared for their meat & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/cow1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/cow2.jpeg}}\\

crib & baby bed with high sides made of slats & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/crib1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/crib2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/crib3.jpeg}}\\

 cup & a container for holding liquids while drinking; includes mugs, and could be made of plastic, glass, ceramic, paper, or styrofoam. Cups include drinking glasses without a stem; if the cup/glass has a stem, it is a wine glass & 
\raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/cup1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/cup2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/cup3.jpeg}}\\

 curtain-other & hanging cloth used as a blind (especially for a window). does not include shower curtains. & 
 \raisebox{-.5\height}{
 \includegraphics[height=1.7cm]{latex/classdefimgs/other-curtain2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/other-curtain1.jpeg}} \\

 desk & A piece of furniture with a flat or sloped surface with drawers, at which one can read, write, or do other work. A table, frame, or case with a sloping or horizontal surface especially for writing and reading and often with drawers, compartments, and pigeonholes. Includes tables used as desks. & 
 \raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/desk5.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/desk2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/desk3.jpeg}} \\

 dishwasher & a machine for washing dishes & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/dishwasher1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/dishwasher2.jpeg}} \\

 dog & a member of the genus Canis (probably descended from the common wolf) that has been domesticated by man since prehistoric times; occurs in many breeds & 
\raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/dog1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/dog2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/dog3.jpeg}} \\

 donut & a small ring-shaped friedcake &
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/donut1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/donut2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/donut3.jpeg}} \\

 door & a swinging or sliding barrier that will close the entrance to a room or building or vehicle & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/door1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/door2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/door3.jpeg}}\\

 elephant & five-toed pachyderm &
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/elephant1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/elephant2.jpeg}} \\

 escalator & a stairway whose steps move continuously on a circulating belt & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/escalator1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/escalator2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/escalator3.jpeg}}\\

 fan & a device for creating a current of air by movement of a surface or surfaces & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/fan4.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/fan1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/fan2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/fan3.jpeg}} \\

 fence & & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/fence1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/fence2.jpeg}}
\\

 fire hydrant & an upright hydrant for drawing water to use in fighting a fire & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/firehydrant1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/firehydrant2.jpeg}} \\

 fireplace & an open recess in a wall at the base of a chimney where a fire can be built & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/fireplace1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/fireplace2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/fireplace3.jpeg}} \\

 flag & emblem usually consisting of a rectangular piece of cloth of distinctive design & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/flag1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/flag2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/flag3.jpeg}} \\

floor & The inside lower horizontal surface (as of a room, hallway, tent, or other structure). Must be indoors. This includes homogenous floor coverings that span an entire room, such as carpet, linoleum, or marble. & 
\raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/floor-example1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/floor-example2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/floor-example3.jpeg}} \\

food\_other & any food that is not a banana, apple, sandwiche, orange, broccoli, carrot, hot\_dog, pizza, donut, cake, or fruit & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/food-other1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/food-other2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/food-other3.jpeg}}\\

fork & cutlery used for serving and eating food & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/fork1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/fork2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/fork3.jpeg}} \\

fountain & an ornamental structure in a pool or lake from which one or more jets of water are pumped into the air. Includes the jet of water. & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/fountain-example-1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/fountain-example-2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/fountain-example-3.jpeg}} \\

frisbee & a light, plastic disk propelled with a flip of the wrist for recreation or competition & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/frisbee1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/frisbee2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/frisbee3.jpeg}} \\

fruit\_other & any fruit not an apple, orange, or banana (e.g. pineapple, melon, pear, kiwi, avocado) & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/fruitother1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/fruitother2.jpeg}} \\

giraffe & tallest living quadruped; having a spotted coat and small horns and very long neck and legs; of savannahs of tropical Africa & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/giraffe1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/giraffe2.jpeg}} \\

gravel & very small rock fragments and pebbles & \\

guard\_rail & a strong fence/railing at the side of a road or in the middle of an expressway, intended to reduce the risk of serious accidents. A guardrail sits low to the ground and is made of thick horizontal metal rails. & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/guardrail3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/guardrail2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/guardrail1.jpeg}} \\

 hair\_dryer & a hand-held electric blower that can blow warm air onto the hair & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/hairdryer1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/hairdryer2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/hairdryer3.jpeg}}\\

 horse & solid-hoofed herbivorous quadruped domesticated since prehistoric times & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/horse1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/horse2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/horse3.jpeg}} \\

 hot dog & a frankfurter served hot on a bun & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/hotdog1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/hotdog2.jpeg}} \\

% & house & & \\
% \hline
 junction box & A metal box outdoors, containing a junction of electric wires or cables & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/junctionbox1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/junctionbox2.jpeg}} \\

 keyboard & a freestanding panel of keys that operate a computer or typewriter. Should not be part of a laptop (to prevent clashes). Connected with a cord to a computer. & 
\raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/keyboard1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/freestanding-keyboard1.jpeg}}
%\includegraphics[height=1.7cm]{latex/classdefimgs/keyboard3.jpeg}
\\

 kitchen-island & an unattached counter in a kitchen that permits access from all sides & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/kitchen-island1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/kitchen-island2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/kitchen-island3.jpeg}} \\

 kite & plaything consisting of a light frame covered with tissue paper; flown in wind at end of a string. Includes kites for windsurfing. & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/kite1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/kite2.jpeg}} \\

 knife & edge tool used as a cutting instrument; has a pointed blade with a sharp edge and a handle & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/knife1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/knife2.jpeg}} \\

 lamp & a device for giving light that has a covering, but allows light to shine through or around. Could be freestanding on a floor and be covered with a shade, or could hang from the ceiling, or be placed on a table/desk/nightstand. & 
\raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/lamp1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/lamp3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/lamp4.jpeg}} \\

 laptop & a portable computer small enough to use in your lap. Includes the laptop keyboard. & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/laptop1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/laptop2.jpeg}} \\

 light-other & Any other type of light, e.g. fluorescent ceiling lights, bathroom lights embedded into ceiling, etc. & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/light-other8.jpg}
\includegraphics[height=1.7cm]{latex/classdefimgs/light-other3.jpg}
\includegraphics[height=1.7cm]{latex/classdefimgs/light-other7.jpg}}
\\

 mailbox & a private box for delivery of mail & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/mailbox2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/mailbox1.jpeg}} \\

 microwave & kitchen appliance that cooks food by passing an electromagnetic wave through it & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/microwave1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/microwave2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/microwave3.jpeg}}\\

 mirror & polished surface that forms images by reflecting light & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/mirror1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/mirror2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/mirror3.jpeg}}\\

 motorcycle & a motor vehicle with two wheels and a strong frame & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/motorcycle1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/motorcycle2.jpeg}} \\

 motorcyclist & a human relying on a motorcycle/moped for movement. Must be actively riding the motorcycle/moped (not standing nearby it). & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/motorcyclist1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/motorcyclist2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/motorcyclist3.jpeg}} \\

 mountain\_hill & & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/mountain-hill1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/mountain-hill2.jpeg}}\\

 mouse & a computer input device that controls an on-screen pointer & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/mouse1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/mouse2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/mouse3.jpeg}}\\

 net & an open fabric of string or rope or wire woven together at regular intervals & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/net1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/net2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/net3.jpeg}} \\

 night stand & a small low bedside table, typically having drawers. a small bedside table or stand & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/nightstand1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/nightstand6.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/nightstand9.jpeg}} \\

 orange & round yellow to orange fruit of any of several citrus trees & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/orange1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/orange2.jpeg}} \\

 ottoman & a low upholstered seat or thick cushion used as a seat & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/ottoman2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/ottoman3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/ottoman4.jpeg}} \\

 oven & & \\

 painting & graphic art consisting of an artistic composition made by applying paints to a surface &
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/painting1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/painting2.jpeg}} \\

 paper & a material made of cellulose pulp derived mainly from wood or rags or certain grasses. Includes loose paper, reams of paper, paper towels, and napkins & 
\raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/paper1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/paper2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/paper3.jpeg}}  \\

 parking meter & a money-operated timer located next to a parking space; depositing money into it entitles you to park your car there for a specified length of time & 
\raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/parkingmeter1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/parkingmeter2.jpeg}} \\

 person\_nonrider & a human being who is not a motorcyclist, bicyclist, or rider\_other  (could be a motor vehicle passenger) & 
\raisebox{-.75\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/person1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/person-nonrider-3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/person-nonrider-1.jpeg}}\\

 pier\_wharf & Either a pier or a wharf. A pier is a platform/low-structure built out from the shore into the water and supported by piles; provides access to ships and boats. A wharf is a level quayside area to which a ship may be moored to load and unload at the edge of water. & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/pier-wharf3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/pier-wharf4.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/pier-wharf1.jpeg}} \\

 pillow & & \\

 pizza & Italian open pie made of thin bread dough spread with a spiced mixture of e.g. tomato sauce and cheese & 
 \raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/pizza1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/pizza2.jpeg}} \\

 plate & &
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/plate1.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/plate2.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/plate3.jpeg}} \\

 platform & area alongside a railway track providing convenient access to trains, or a ramp/raised surface at a skatepark & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/platform1.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/platform3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/platform4.jpeg}} \\

playingfield & a field used for outdoor team games. Includes tennis courts, baseball fields/diamonds, and fields for soccer, ultimate frisbee, and equestrian events. & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/plaything6.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/playingfield1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/playingfield2.jpeg}} \\

 plaything\_other & a child's toy, or something used like a toy, that is not a teddy bear. & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/plaything6.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/plaything4.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/plaything2.jpeg}} \\

 pole & a long (usually round) rod of wood or metal or plastic. includes lamp posts (excluding the light) and streetlight poles (excluding the light) & \\

 pool table & game equipment consisting of a heavy table on which pool is played & 
 \raisebox{-.5\height}{
 \includegraphics[height=1.7cm]{latex/classdefimgs/pooltable1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/pooltable2.jpeg}} \\

 poster & & \\

 potted plant & a plant that is planted and grown in a container rather than in the ground & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/pottedplant1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/pottedplant2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/pottedplant3.jpeg}} \\
 \\

 radiator & heater consisting of a series of pipes for circulating steam or hot water to heat rooms or buildings & 
\raisebox{-.5\height}{\includegraphics[height=1.7cm]{latex/classdefimgs/radiator1.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/radiator2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/radiator3.jpeg}} \\

 railing-banister & a barrier consisting of a horizontal bar and supports; a railing at the side of a staircase or balcony to prevent people from falling & \\

 railroad & a line of track providing a runway for wheels & 
  \raisebox{-.5\height}{
 \includegraphics[height=1.7cm]{latex/classdefimgs/railroad1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/railroad2.jpeg}} \\

 range\_hood & exhaust hood over a kitchen range & 
  \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/rangehood1.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/rangehood2.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/rangehood3.jpeg}} \\

 refrigerator & a refrigerator in which the coolant is pumped around by an electric motor & 
  \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/refridgerator1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/refridgerator2.jpeg}}\\

 remote &  a device that can be used to control a machine or apparatus from a distance &
  \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/remote2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/remote1.jpeg}} \\

 rider\_other & a human relying upon a segway, skateboards, electric scooter, lawn mower, rickshaw, wheelchair etc (any other device that is not a motorcycle, bicycle, or vehicle) for movement on land. &
  \raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/other-rider1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/other-rider2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/other-rider3.jpeg}}\\

 river\_lake & River or lake. River: a large natural stream of water, with possible rapids. Lake: a body of (usually fresh) water surrounded by land. Lakes generally have very still water. Should appear naturally formed. &
  \raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/riverlake1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/riverlake2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/riverlake3.jpeg}} \\

 road & a long, narrow stretch with a smoothed or paved surface, made for traveling by motor vehicle, between two or more points; street or highway. Often bounded by curbs. & 
\raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/road2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/road3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/road4.jpeg}} \\

 road\_barrier & concrete safety barriers on roads and highways; also known as Jersey barrier & 
 \raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/roadbarrier1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/roadbarrier2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/roadbarrier3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/roadbarrier4.jpeg}} \\

 rock & a lump or mass of hard consolidated mineral matter & 
  \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/rock1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/rock2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/rock3.jpeg}}\\

 rug\_floormat & a floor covering of thick woven material or animal skin -- just with limited size, covers only a small section of the floor. Includes rugs, and floor mats (door mats, bath mat). Does not include carpet. & 
  \raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/rugfloormat3}
\includegraphics[height=1.7cm]{latex/classdefimgs/rugfloormat2}
\includegraphics[height=1.7cm]{latex/classdefimgs/rugfloormat1}}\\

runway & a strip of level paved surface where planes can take off, land, or taxi from a terminal; or a narrow platform extending from the stage into the audience in a theater or nightclub etc. & 
 \raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/runwaydefn1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/runwaydefn2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/runwaydefn3.jpeg}}\\

 sandwich & two (or more) slices of bread with a filling between them & 
 \raisebox{-.5\height}{
 \includegraphics[height=1.7cm]{latex/classdefimgs/sandwich1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/sandwich2.jpeg}} \\

 scissors & an edge tool having two crossed pivoting blades &
  \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/scissors1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/scissors2.jpeg}} \\

 sconce & a decorative wall bracket/object for holding lightbulbs, candles or other sources of light. Must be attached to the side of a wall.  & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/sconce3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/sconce1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/sconce9.jpg}} \\

 sculpture & statue or a three-dimensional work of art & 
  \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/sculpture1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/sculpture2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/sculpture3.jpeg}} \\

 sea & A sea or ocean. Often has large amounts of waves/surf and a sandy beach. May have surfers on surfboards. Unlike a river or a lake, one generally cannot see the far bank of a sea/ocean. & 
 \raisebox{-.75\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/sea1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/sea2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/sea3.jpeg} }\\

seat & a space reserved for sitting (as in a theater, auditorium, stadium, on a train or airplane, or in a car). (that is not a bench, chair, stool, sofa, or armchair) & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/seat1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/seat2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/seat3.jpeg}} \\
\\

sheep & woolly usually horned ruminant mammal related to the goat & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/sheep1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/sheep2.jpeg}} \\

shelf & & \\

shower & & \\

shower\_curtain & fabric found next to a bathtub or shower to keep water from spilling out into the bathroom &
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/showercurtain2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/showercurtaindefn3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/showercurtaindefn1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/showercurtaindefn2.jpeg}} \\

sidewalk\_pavement & walk consisting of a paved area for pedestrians; usually beside a street or roadway (not a road) & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/pavement_sidewalk4.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/pavement_sidewalk1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/pavement_sidewalk2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/pavement_sidewalk3.jpeg}}\\

sink & plumbing fixture consisting of a water basin fixed to a wall or floor and having a drainpipe (usually in a bathroom or kitchen) &
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/sink2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/sink1.jpeg}} \\

 skateboard & a board with wheels that is ridden in a standing or crouching position and propelled by foot &
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/skateboard2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/skateboard1.jpeg}} \\

 skis & sports equipment for skiing on snow & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/skis1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/skis2.jpeg}} \\

sky & the atmosphere and outer space as viewed from the earth & \\

slow wheeled object & any slow-moving wheeled object, such as strollers, wheelchairs, and carts & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/slow_wheeled1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/slow_wheeled2.jpeg}} \\

snow & a layer of snowflakes (white crystals of frozen water) covering the ground & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/snow1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/snow2.jpeg}} \\

snowboard & a board that resembles a broad ski or a small surfboard; used in a standing position to slide down snow-covered slopes &
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/snowboard1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/snowboard2.jpeg}} \\

spoon & a piece of cutlery with a shallow bowl-shaped container and a handle; used to stir or serve or take up food &
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/spoon1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/spoon2.jpeg}} \\

 sports\_ball & round object that is hit or thrown or kicked in games & 
  \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/sportsball3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/sportsball4.jpeg}} \\

 stage & a large platform on which people can stand and can be seen by an audience & 
  \raisebox{-.5\height}{
 \includegraphics[height=1.7cm]{latex/classdefimgs/stage1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/stage2.jpeg}} \\

 stairs & & \\

 stool & a simple seat without a back or arms; or a high seat at a bar without arms & 
  \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/stool1.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/stool3.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/stool4.jpeg}} \\

storage\_tank & a large (usually metallic) vessel for holding gases or liquids & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/tank1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/tank2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/tank3.jpeg}} \\

 stove & & 
   \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/stove1.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/stove2.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/stove3.jpeg}} \\

 streetlight & a lamp or light supported on a lamppost/pole; for illuminating a street & 
  \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/streetlight1.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/streetlight2.jpeg} 
\includegraphics[height=1.7cm]{latex/classdefimgs/streetlight3.jpeg}}\\

 suitcase & a portable rectangular container for carrying clothes &
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/suitcase1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/suitcase2.jpeg}}\\

 surfboard & a narrow buoyant board for riding surf &
 \raisebox{-.5\height}{
 \includegraphics[height=1.7cm]{latex/classdefimgs/surfboard1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/surfboard2.jpeg}} \\

 swimming\_pool & pool that provides a facility for swimming & 
 \raisebox{-.5\height}{
 \includegraphics[height=1.7cm]{latex/classdefimgs/swimmingpool1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/swimmingpool2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/swimmingpool3.jpeg}
}\\

swivel\_chair & a chair that swivels on its base. Can be turned around a central point to face in a different direction without moving the legs &
 \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/swivel-chair1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/swivel-chair3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/swivel-chair4.jpeg}} 
\\

 table & A piece of furniture consisting of a smooth flat slab fixed on legs. A piece of furniture with a flat top and one or more legs, providing a level surface on which objects may be placed, and that can be used for such purposes as eating, writing, working, or playing games. & 
  \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/table3.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/table4.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/table5.jpeg}} \\

 teddy\_bear & Stuffed toy in the form of a bear. It is a type of plaything/child's toy (usually plush and stuffed with soft materials). & 
   \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/teddybear1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/teddybear2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/teddybear3.jpeg}} \\

 television & & \\

 tennis racket & a racket used to play tennis &
   \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/tennisracket1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/tennisracket2.jpeg}} \\

 tent & a portable shelter (usually of canvas stretched over supporting poles and fastened to the ground with ropes and pegs). For example, a camping tent. & 
  \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/tent2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/tent1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/tent3.jpeg}} \\

 terrain & dirt, sand, grass, or any kind of horizontally spreading vegetation & \\

 tie & neckwear consisting of a long narrow piece of material worn (mostly by men) under a collar and tied in knot at the front & 
  \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/tie1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/tie2.jpeg}}\\

 toaster & & 
  \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/toaster1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/toaster2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/toaster3.jpeg}} \\

 toilet & a plumbing fixture for defecation and urination & 
  \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/toilet1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/toilet2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/toilet3.jpeg}} \\

 toothbrush & small brush; has long handle; used to clean teeth &
  \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/toothbrush2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/toothbrush1.jpeg}} \\

 towel & a thick, rectangular piece of absorbent cloth for drying or wiping & \\

 traffic light & a visual signal to control the flow of traffic at intersections (includes stoplights, pedestrian crossing lights, etc) &
  \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/trafficlight1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/trafficlight2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/trafficlight3.jpeg}} \\

 traffic sign & a sign usually on the side of a street or highway bearing symbols or words of warning or direction to motorists or pedestrians & 
\raisebox{-.75\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/trafficsign2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/trafficsign1.jpeg}} \\
 \hline
 trailer & & \\

 train & All vehicles that move on rails, e.g. trams, trains. &
  \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/train1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/train2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/train3.jpeg}} \\

 trash can & a bin that holds rubbish until it is collected &
 \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/trashcan1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/trashcan2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/trashcan3.jpeg}}\\

 tray & a flat, shallow container with a raised rim, typically used for carrying food and drink, or for holding small items. &
  \raisebox{-.5\height}{ 
 \includegraphics[height=1.7cm]{latex/classdefimgs/tray1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/tray2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/tray3.jpeg}} \\

 truck & & \\

tunnel & a passageway through or under something, usually underground (especially one for trains or cars) & 
 \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/tunnel1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/tunnel2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/tunnel3.jpeg}} \\

 umbrella & a lightweight collapsible canopy. Could be handheld or mounted above a table outdoors. & 
  \raisebox{-.5\height}{ 
 \includegraphics[height=1.7cm]{latex/classdefimgs/umbrella1.jpeg}
 \includegraphics[height=1.7cm]{latex/classdefimgs/umbrella2.jpg}}\\

vase & an open jar of glass, porcelain, or metal used as an ornament or to hold flowers & 
 \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/vase1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/vase2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/vase3.jpeg}} \\

 vegetation & Trees, hedges, and all kinds of vertically growing vegetation (for example, must be higher than lawn grass) & 
 \raisebox{-.5\height}{ 
\includegraphics[height=1.7cm]{latex/classdefimgs/vegetation1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/vegetation2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/vegetation3.jpeg}} \\

 wall & Either: one of the sides of a room or building connecting floor and ceiling. Or: a masonry fence around a garden, park, or estate. & 
\raisebox{-.75\height}{ 
 \includegraphics[height=1.7cm]{latex/classdefimgs/wall0.jpeg} \includegraphics[height=1.7cm]{latex/classdefimgs/wall1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/wall2.jpeg}} \\

wardrobe & a tall piece of furniture that provides storage space for clothes; has a door and rails or hooks for hanging clothes & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/wardrobe-example-6.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/wardrobe-example-1.jpeg}} \\

 washer-dryer & a home appliance for washing or drying clothes and linens automatically & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/washingmachine1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/washingmachine2.jpeg}} \\

waterfall & a steep descent of the water of a river & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/waterfall1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/waterfall2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/waterfall3.jpeg}
}\\

 water\_other & all other kinds of water, e.g. puddles, ditchwater, aquariums, shallow artificially made ponds, zoo ponds, flooded areas, bathtub water, water coming out of a fire hydrant, water from a kitchen faucet, etc. Is not a lake,  river, fountain, swimming pool, or sea. &
 \raisebox{-.75\height}{
 \includegraphics[height=1.7cm]{latex/classdefimgs/water-other1.jpeg} 
 \includegraphics[height=1.7cm]{latex/classdefimgs/water-other2.jpeg} 
 \includegraphics[height=1.7cm]{latex/classdefimgs/water-other4.jpeg}
 }\\

% \hline
 whiteboard & a hard smooth white surface used for writing or drawing on with markers. & 
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/whiteboard1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/whiteboard2.jpeg} 
}\\

 window & a framework of wood or metal that contains a glass windowpane and is built into a wall or roof to admit light or air & 
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/window1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/window2.jpeg}} \\

 window-blind & A blind for privacy or to keep out light. Placed indoors on a window. &
 \raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/windowblind1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/windowblind2.jpeg}} \\

 wine\_glass & a glass that has a stem and in which wine is served &
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/wineglass1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/wineglass2.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/wineglass3.jpeg}} \\

 zebra & any of several fleet black-and-white striped African equines &
\raisebox{-.5\height}{
\includegraphics[height=1.7cm]{latex/classdefimgs/zebra1.jpeg}
\includegraphics[height=1.7cm]{latex/classdefimgs/zebra2.jpeg}} \\
\bottomrule
\end{longtable}
\twocolumn
\normalsize
\renewcommand{\thefootnote}{\arabic{footnote}}
\renewcommand{\arraystretch}{1.0}
% \end{portrait}




==> tex/eval_relabeled_data.tex <==


%In this discussion, we discuss the fair evaluation of trained models' performance on the validation split of MSeg's relabeled component training datasets. For example, does relabeling COCO improve a model's performance on ADE20k? This evaluation is nontrivial, since the notion of ground truth differs in two cases. For example, a model $\mathcal{M}_{unrel}$ trained on COCO's original ground truth $L_{gt\_unrel}$ will have no sense of ``motorcyclist'' and will predict a motorcycle rider in a COCO image as ``person'', which matches the original ground truth $L_{gt\_unrel}$, but achieves zero IoU when compared with re-labeled data $L_{gt\_rel}$. This is clearly unfair. However, on the other hand, a model $\mathcal{M}_{rel}$ trained on relabeled COCO, will predict such an entity as a ``motorcyclist'', matching the relabeled ground truth $L_{gt\_rel}$. If $\mathcal{M}_{rel}$ is evaluated on $L_{gt\_unrel}$, it will obtain a zero score for its correct prediction, which is also unfair. Clearly 

%Thus, we must find a way to fairly evaluate the models trained on the original, unrelabeled data. For shattered classes, converting all relabeled label maps $L_{gt\_rel}$ to their unrelabeled state $L_{gt\_unrel}$ is straightforward and can be performed globally at the taxonomic level. This is because  for shattered classes, the process only involves replacing children nodes with their parent. For example, for another motorcylist image in Cityscapes, when a `rider' is relabeled to one of  $\{$`bicyclist',`motorcyclist', `rider-other'$\}$, if the unrelabeled MSeg model $\mathcal{M}_{unrel}$ predicts `rider', it is correct. In other words, the shattering is relaxed. 

%For classes with directed acyclic graph (DAG structure), global taxonomic rules are impossible, and per-pixel rules are required. A single parent (inverse in the map) no longer exists for such classes. For example, COCO Panoptic's ``cabinet-merged'' and ``table-merged'' with near equal probability could be relabeled as ``nightstand'', leaving a leaf node with two parents (See Figure 2G of the main paper). A remapping rule is defined for only a single mask, i.e. its pixels.


%While we could also proceed in the opposite direction, evaluating $\mathcal{M}_{unrel}$ on $\mathcal{L}_{rel}$ via pixel remapping, this is not preferred. To proceed in the opposite direction, we need human-annotated pixel supervision, since three children nodes of `rider' exist and it is unknown a priori which is correct. If the relabeled MSeg model $\mathcal{M}_{rel}$ predicts `motorcyclist', it is also correct, although it had a more challenging and fine-grained decision to make. 

%Specifically, evaluating $\mathcal{M}_{rel}$ on $L_{gt\_unrel}$ is preferred since it is closer to the original taxonomy. Although we train all training-dataset model baselines in a 194-class universal taxonomy $\mathcal{T}_{unified}$, thus the taxonomy already differs from the original 19 Cityscapes classes, there is a 1:1 correspondence between 19 $\mathcal{T}_{unified}$ categories and $\mathcal{T}_{Cityscapes}$ categories, therefore we can compute mIoU over their intersection (19 categories), making this evaluation method comparable with the literature.  $L_{gt\_rel}$ relies upon $\mathcal{T}_{Cityscapes-relabeled}$, and thus has 21 categories.

%We implement the evaluation of $\mathcal{M}_{rel}$ on $L_{unrel}$ as a function $f$ with three arguments: $f: \mathcal{M}_{rel} \times L_{gt\_unrel} \times L_{gt\_rel}$. If $\mathcal{M}_{rel}$ makes a prediction $P$,  check for correct locations $\mathcal{C}=\{c_{ij}\}$ 
%\begin{equation}
% \mathcal{C} = \{ (i,j): P_{ij} = L_{{gt\_rel}_{ij}} \}
%\end{equation}
%We next identify relabeled locations $\mathcal{R} = \{r_{ij}\}$ as:
%\begin{equation}
% \mathcal{R} = \{ (i,j): L_{{gt\_unrel}_{ij}} \neq L_{{gt\_rel}_{ij}} \}
%\end{equation}
%We implement a symmetric reward and penalty to update the predicted label map $P$ to $P_{updated}$. Where $P$ matches $L_{gt\_rel}$, we provide a reward by replacing the pixel's category with the corresponding inverse in $L_{gt\_unrel}$:
%\begin{equation}
    %P_{updated} := \begin{cases} L_{gt\_unrel} & \mbox{if } c_{ij} \odot %r_{ij} = 1 \\ NULL & \mbox{else if } c_{ij} \odot r_{ij} \neq 1
%    \end{cases}
%\end{equation}
%where $NULL$ will generate zero IoU for the pixel of interest.


==> tex/grid-figure.tex <==
\begin{figure*}
	\centering
	\small
	\begin{tabular}{@{\hspace{0.0mm}}c@{\hspace{1.0mm}}c@{\hspace{1.0mm}}c@{\hspace{2.5mm}}c@{\hspace{1.0mm}}c@{\hspace{1.0mm}}c@{\hspace{0.0mm}}}
		Input & Ground Truth & Unified Model & Input & Ground Truth & Unified Model\\
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}\\
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}\\
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}\\
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth]{figure/results/snapshot00.png}\\
		\includegraphics[width=0.16\linewidth, height=18.5mm]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth, height=18.5mm]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth, height=18.5mm]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth, height=18.5mm]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth, height=18.5mm]{figure/results/snapshot00.png}&
		\includegraphics[width=0.16\linewidth, height=18.5mm]{figure/results/snapshot00.png}\\
		%\multicolumn{6}{c}{\includegraphics[width=0.9\linewidth]{figure/colorbar.pdf}}\\
	\end{tabular}
	\caption{Visualization of semantic segmentation results on each dataset.}
	\label{fig:qual-visual}
\end{figure*}
